Enhancing Robustness in Manipulability Assessment: The Pseudo-Ellipsoid Approach

Manipulability analysis is a methodology employed to assess the capacity of an articulated system, at a specific configuration, to produce motion or exert force in diverse directions. The conventional method entails generating a virtual ellipsoid using the system's configuration and model. Yet, this approach poses challenges when applied to systems such as the human body, where direct access to such information is limited, necessitating reliance on estimations. Any inaccuracies in these estimations can distort the ellipsoid's configuration, potentially compromising the accuracy of the manipulability assessment. To address this issue, this article extends the standard approach by introducing the concept of the manipulability pseudo-ellipsoid. Through a series of theoretical analyses, simulations, and experiments, the article demonstrates that the proposed method exhibits reduced sensitivity to noise in sensory information, consequently enhancing the robustness of the approach.

==> packages.tex <==
% ------------------------------------------------------------------
%
%  Usedpaclages and macros
%
% ------------------------------------------------------------------
\usepackage{etex} % this must be the first loaded package

\ifx\isieee % if isieee is not defined
	\usepackage{lmodern}
	\usepackage{titlesec}
	\usepackage{amsfonts}
	\usepackage[T1]{fontenc} 
\else
	
\fi

% ---------------------------------------------------------------------
%  packages
% ---------------------------------------------------------------------
\usepackage{lipsum}
\usepackage[makeroom]{cancel}
\usepackage{subcaption}
\usepackage{textgreek} % for Greek in Ergos
\usepackage{xcolor}
\usepackage{tikz}
\usepackage[compress]{cite}
\usepackage[utf8]{inputenc}
\usepackage{makeidx}
\usepackage{amsmath,bm}
\newcommand\inlineeqno{\refstepcounter{equation}\ (\theequation)}
\usepackage{amsbsy}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{color}
\usepackage{ifpdf}
\usepackage{wrapfig}
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{sidecap}
\usepackage[]{threeparttable}
\usepackage[table]{xcolor}
\usepackage{tabularx}
\usepackage{multirow}
\usepackage{relsize}
%\usepackage[chapter]{algorithm}
\usepackage{algorithm}
\usepackage{algorithmic}
\renewcommand{\algorithmiccomment}[1]{ {\hfill \scriptsize//~#1\normalsize} }
\usepackage{pgfplots}
\usepackage{mathrsfs}
\usepackage{bbm}
%\usepackage{china2e}
\usepackage{mathtools}
\usepackage{enumitem}
\usepackage{upgreek}
\usepackage{trfsigns}
\usepackage{arcs}
\usepackage{pgf}
\usepackage{tikz}
\usepackage{lscape}
\usepackage{dblfloatfix} 
\usetikzlibrary{shapes.geometric,arrows.meta,automata,positioning,backgrounds}
\usepackage[figuresright]{rotating}
\usepackage[stable, hang]{footmisc}
\usepackage{xparse,mathtools}
\usepackage{xstring}
\setlength\footnotemargin{10pt}
\setlist{leftmargin=3.25ex,itemsep=0ex}
\ifpdf
  \DeclareGraphicsExtensions{.pdf,.jpg,.png,.ps,.eps}
\else
  \DeclareGraphicsExtensions{.eps,.ps,.png,.jpg,.pdf}
\fi
\renewcommand{\thealgorithm}{\thechapter.\arabic{algorithm}} 
\usepackage[normalem]{ulem}
\setcounter{MaxMatrixCols}{20}
%\titleformat*{\paragraph}{\sffamily\small\bfseries}
\DeclareMathAlphabet{\mathbfsf}{\encodingdefault}{\sfdefault}{bx}{sl}
\DeclareMathAlphabet{\mathitsf}{\encodingdefault}{\sfdefault}{m}{sl}
% ---------------------------------------------------------------------
%  hyperref package
% ---------------------------------------------------------------------
\ifpdf
  \usepackage{hyperref}
\else
  \usepackage[hypertex]{hyperref}
\fi
\definecolor{dgreen}{rgb}{0,0.7,0}
\definecolor{ddgreen}{rgb}{0,0.5,0}
\definecolor{dblue}{rgb}{0,0,0.7}
\definecolor{dred}{rgb}{0.7,0,0}
\hypersetup{bookmarksnumbered=true,
            plainpages=false,
            colorlinks=true,
            linkcolor=dblue,
            citecolor=dgreen,
            filecolor=dred,
            urlcolor=blue}

% cross-reference and theorems
\ifx\isieee % if isieee is not defined
	\newcommand{\figref}[1]{Figure~\ref{#1}}
	\newcommand{\tabref}[1]{Table~\ref{#1}}
	\renewcommand{\eqref}[1]{(\ref{#1})}
	\newcommand{\theoremref}[1]{Theorem~\ref{#1}}
	\newcommand{\sysref}[1]{System~(\ref{#1})}
\else
	\newcommand{\figref}[1]{Fig.~\ref{#1}}
	\newcommand{\tabref}[1]{Table~\ref{#1}}
	%\renewcommand{\eqref}[1]{(\ref{#1})}
	\newcommand{\sysref}[1]{System~(\ref{#1})}
	%
	\newtheorem{definition}{Definition}
	\newtheorem{theorem}{Theorem}
	\newtheorem{lemma}{Lemma}
	\newcommand{\theoremref}[1]{Theorem~\ref{#1}}
	\newcommand{\lemmaref}[1]{Lemma~\ref{#1}}
\fi
\captionsetup[figure]{justification=justified,singlelinecheck=false}

% author comments
\newcommand{\hu}[1]{\textcolor{red}{[Hu: #1]}}
\newcommand{\kn}[1]{\textcolor{red}{[K\"{u}hn:#1]}}
\newcommand{\haddadin}[1]{\textcolor{red}{[{Haddadin: #1}]}}
%\newcommand{\herleitung}[1]{\textcolor{blue}{[{Hu: #1}]}}
\newcommand{\herleitung}[1]{\textcolor{blue}{}}


% finite state machine
\tikzstyle{startstop} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm,text centered, draw=black, thick, fill=red!30]
\tikzstyle{io} = [trapezium, trapezium left angle=70, trapezium right angle=110, minimum width=3cm, minimum height=1cm, text centered, draw=black, thick, fill=blue!30]
\tikzstyle{process} = [rectangle, minimum width=3cm, minimum height=1cm, text centered, draw=black, thick, fill=orange!30]
\tikzstyle{decision} = [diamond, aspect=3, minimum width=3cm, minimum height=1cm, text centered, draw=black, thick, fill=green!30]
\tikzstyle{arrow} = [thick,->,>=stealth]
\tikzstyle{noarrow} = [thick,-]
\tikzstyle{doublearrow} = [thick, double distance=1pt, ->, >=stealth]
\tikzstyle{doublenoarrow} = [thick, double distance=1pt]
\tikzstyle{outerwhite} = [thin, white, line width=5pt, shorten >= 4.5pt]
\tikzstyle{innerwhite} = [thin, white, line width=1pt]
%\tikzstyle{null} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm,text centered, draw=white]
\tikzset{state/.style={
           rectangle,
           rounded corners,
           draw=black, very thick,
           minimum height=2em,
           inner sep=2pt,
%           text centered,
           },}
\tikzstyle{start} = [circle, inner sep=0.06cm, draw=black, fill=black]      

% block diagram
\tikzstyle{gain} = [draw, very thick, fill=white, regular polygon, regular polygon sides=3, shape border rotate=30, minimum height=3em, minimum width=3em, align=center]
%
\tikzstyle{bigblock} = [draw, thick, fill=white, rectangle, 
minimum height=4em, minimum width=6em, align=center]
\tikzstyle{smallblock} = [draw, thick, fill=white, rectangle, 
minimum height=1em, minimum width=1em, align=center]
\tikzstyle{medianblock} = [draw, thick, fill=white, rectangle, 
minimum height=3em, minimum width=3em, align=center]
%
\tikzstyle{bigfcnblock} = [draw, thick, fill=white, rectangle, 
minimum height=4em, minimum width=6em, double, double distance=0.5mm, align=center]
\tikzstyle{smallfcnblock} = [draw, thick, fill=white, rectangle, 
minimum height=1em, minimum width=1em, double, double distance=0.5mm, align=center]
\tikzstyle{medianfcnblock} = [draw, thick, fill=white, rectangle, 
minimum height=3em, minimum width=3em, double, double distance=0.5mm, align=center]
%
\tikzstyle{invisiblenode} = [draw=none, minimum size=0pt, align=center]
\tikzstyle{sum} = [draw, thick, fill=white, circle, node distance=1cm]
\makeatletter
\pgfdeclareshape{record}{
	\inheritsavedanchors[from={rectangle}]
	\inheritbackgroundpath[from={rectangle}]
	\inheritanchorborder[from={rectangle}]
	\foreach \x in {center,north east,north west,north,south,south east,south west}{
		\inheritanchor[from={rectangle}]{\x}
	}
	\foregroundpath{
		\pgfpointdiff{\northeast}{\southwest}
		\pgf@xa=\pgf@x \pgf@ya=\pgf@y
		\northeast
		\pgfpathmoveto{\pgfpoint{0}{0.33\pgf@ya}}
		\pgfpathlineto{\pgfpoint{0}{-0.33\pgf@ya}}
		\pgfpathmoveto{\pgfpoint{0.33\pgf@xa}{0}}
		\pgfpathlineto{\pgfpoint{-0.33\pgf@xa}{0}}
		\pgfpathmoveto{\pgfpointadd{\southwest}{\pgfpoint{-0.33\pgf@xa}{-0.6\pgf@ya}}}
		\pgfpathlineto{\pgfpointadd{\southwest}{\pgfpoint{-0.5\pgf@xa}{-0.6\pgf@ya}}}
		\pgfpathlineto{\pgfpointadd{\northeast}{\pgfpoint{-0.5\pgf@xa}{-0.6\pgf@ya}}}
		\pgfpathlineto{\pgfpointadd{\northeast}{\pgfpoint{-0.33\pgf@xa}{-0.6\pgf@ya}}}
	}
}
\makeatother
\tikzstyle{saturation} = [draw, record, fill=white, minimum height=3em, minimum width=3em]

% mechanics
\tikzstyle{spring}=[thick,decorate,decoration={zigzag,amplitude=0.2cm,pre length=0.3cm,post length=0.3cm,segment length=6}]
\tikzstyle{damper}=[thick,decoration={markings,  
  mark connection node=dmp,
  mark=at position 0.5 with 
  {
    \node (dmp) [thick,inner sep=0pt,transform shape,rotate=-90,minimum width=15pt,minimum height=3pt,draw=none] {};
    \draw [thick] ($(dmp.north east)+(2pt,0)$) -- (dmp.south east) -- (dmp.south west) -- ($(dmp.north west)+(2pt,0)$);
    \draw [thick] ($(dmp.north)+(0,-5pt)$) -- ($(dmp.north)+(0,5pt)$);
  }
}, decorate]
\tikzstyle{ground}=[fill,pattern=north east lines,draw=none,minimum width=0.75cm,minimum height=0.3cm]

% vectors
\tikzset{
	pics/.cd,
	vector out/.style={
		code={
			\draw[#1] (0,0)  circle (1) (45:1) -- (225:1) (135:1) -- (315:1);
		}%end code   
	}%end style
}%end tikzset
\tikzset{
	pics/.cd,
	vector in/.style={
		code={
			\draw[#1] (0,0)  circle (1);
			\fill[#1] (0,0)  circle (.1);
		}%end code   
	}%end style
}%end tikzset

% robots


% others
\pgfdeclarelayer{bg}    % declare background layer
\pgfsetlayers{bg,main}  % set the order of the layers (main is the standard layer)
\tikzstyle{circlenode} = [draw, circle, minimum width=1pt]
\newcommand{\midarrow}{\tikz \draw[-triangle 90] (0,0) -- +(.1,0);}

\tikzstyle{hexagonnode} = [draw, thick, shape=regular polygon, regular polygon sides=6, minimum width=5pt]

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
		\node[shape=circle,draw,inner sep=2pt] (char) {#1};}}

% redefine derivatives
\newcommand\scaleddot{\scalebox{.89}{.}}
\makeatletter
\renewcommand{\dddot}[1]{%
	{\mathop{\kern\z@#1}\limits^{\makebox[0pt][c]{\vbox to-1.7\ex@{\kern-\tw@\ex@
					\hbox{\normalfont\scaleddot\kern-0.5pt\scaleddot\kern-0.5pt\scaleddot}\vss}}}}}
\renewcommand{\ddddot}[1]{%
	{\mathop{\kern\z@#1}\limits^{\makebox[0pt][c]{\vbox to-1.7\ex@{\kern-\tw@\ex@
					\hbox{\normalfont\scaleddot\kern-0.5pt\scaleddot\kern-0.5pt\scaleddot\kern-0.5pt\scaleddot}\vss}}}}}
\makeatother

==> sections/kim_ideas.tex <==


%
% OR somthing like this
%manipulability of articulated body, such as the human arm or a robot manipulator can serve to evaluate whether the arm's configuration is appropriate for a given task at hand on kinematic level.. 

Towards increased Ergonomic Manipulation Feedback: The Pseudo-Ellipsoid Approach

Ensuring Ergonomic Manipulability in Human-Robot Interaction: The Pseudo-Ellipsoid Approach

Towards Increased Ergonomic Human Manipulability: The Pseudo-Ellipsoid Approach

Towards Increased Ergonomic Manipulability: The Pseudo-Ellipsoid Approach

--> Erfan
- Transferring from robots to humans
- Assessment of ... for human manipulability 
- Assessing human manipulability with increased robustness (or decreased sensitivity)
- A robust way of assessing human manipulability 
- low-cost equipment / 
- more people can use the manipulability 
- easier access to tracking 
- 

%just some ideas from me from the other paper 
%could go in the discussion maybe+

Robot manipulation is always a research hot spot since late twenties. It reflects the robot posture and feasible working space, and greatly influence the application of robots in the industry and daily life. With an optimal manipulability, the robot can finish a task with less effort, more reasonable trajectory and lots of other benefits. This is of particular interest in the field of HRI, as the robot should act as a partner and supporter of the human being. Therefore, it is interesting to take a closer look at how the manipulability of the robot can be optimized and which data information is of great value for this purpose. There are different methods of manipulability measurement like manipulability polytopes and manipulability ellipsoid which were first introduced in ~\cite{}.
The velocity manipulability ellipsoid, derived from forward kinematic model (FKM), is one of the most commonly used manipulability measurement nowadays.
When looking at humans, most tasks are done "easily", smooth".... but when it comes to HRI, e.g. teaching a robot a task, the movement can become quite unnaturally while adapting to the robots manipulability. Therefore, the robot is not a supporter or even a partner in a task. To change this, may we need to think how the robot can learn to adapt to the human manipulability ellipsoid when getting taught and even perceives the motion of the human.
help, support, assist
%-------------------

Unergonomic joint configurations during lifting tasks,..., can cause msucle and joint problems/ pain as also reported in....

Beside that, 
